Aggregation-Based Certificate Transparency Gossip

Certificate Transparency (CT) requires that every CA-issued TLS certificate must be publicly logged. While a CT log need not be trusted in theory, it relies on the assumption that every client observes and cryptographically verifies the same log. As such, some form of gossip mechanism is needed in practice. Despite CT being adopted by several major browser vendors, no gossip mechanism is widely deployed. We suggest an aggregation-based gossip mechanism that passively observes cryptographic material that CT logs emit in plaintext, aggregating at packet processors (such as routers and switches) to periodically verify log consistency off-path. In other words, gossip is provided as-a-service by the network. Based on 20 days of RIPE Atlas measurements that represent clients from 3500 autonomous systems and 40% of the IPv4 space, our proposal can be deployed incrementally for a realistic threat model with significant protection against split-viewing CT logs. We also show that aggregation-based gossip can be implemented for a variety of packet processors using P4 and XDP, running at 10 Gbps line-speed.

==> src/keywords.tex <==
Certificate Transparency \and
Programmable data planes \and
Gossip.

